Teaching Broad Reasoning Skills for Multi-Step QA by Generating Hard Contexts

Question-answering datasets require a broad set of reasoning skills. We show how to use question decompositions to teach language models these broad reasoning skills in a robust fashion. Specifically, we use widely available QDMR representations to programmatically create hard-to-cheat synthetic contexts for real questions in six multi-step reasoning datasets. These contexts are carefully designed to avoid reasoning shortcuts prevalent in real contexts that prevent models from learning the right skills. This results in a pretraining dataset, named TeaBReaC, containing 525K multi-step questions (with associated formal programs) covering about 900 reasoning patterns. We show that pretraining standard language models (LMs) on TeaBReaC before fine-tuning them on target datasets improves their performance by up to 13 F1 points across 4 multi-step QA datasets, with up to 21 point gain on more complex questions. The resulting models also demonstrate higher robustness, with a 5-8 F1 point improvement on two contrast sets. Furthermore, TeaBReaC pretraining substantially improves model performance and robustness even when starting with numerate LMs pretrained using recent methods (e.g., PReasM, POET). Our work thus shows how to effectively use decomposition-guided contexts to robustly teach multi-step reasoning.

==> tables/digit-tokenization.tex <==
\begin{table}[ht]
    \centering
    \small
    \setlength{\tabcolsep}{1.5pt}
    \begin{tabular}{p{5.4cm}cc}\toprule
        Method      & Dig. Tok. & DROP \\

        \midrule
        T5 (reported in ~\cite{preasm})     &  \faTimes  &  61.8 \\
        % T5 (our implementation)             &  \faTimes  &  xx.x \\
        T5 (our implementation)             &  \faCheck  &  \textbf{70.3} \\

        \midrule
        PReasM (reported in ~\cite{preasm})     &  \faTimes  &  69.4 \\
        % PReasM (our implementation)             &  \faTimes  &  xx.x \\
        PReasM (our implementation)             &  \faCheck  &  \textbf{76.6} \\

        \bottomrule
    \end{tabular}
    \caption{Digit tokenization (character tokenization for numbers) significantly helps downstream performance, so we use it for all models.}
    \label{table:digit-tokenization}
\end{table}
